Slightly Conservative Bootstrap for Maxima of Sums

We study the bootstrap for the maxima of the sums of independent random variables, a problem of high relevance to many applications in modern statistics. Since the consistency of bootstrap was justified by Gaussian approximation in Chernozhukov et al. (2013), quite a few attempts have been made to sharpen the error bound for bootstrap and reduce the sample size requirement for bootstrap consistency. In this paper, we show that the sample size requirement can be dramatically improved when we make the inference slightly conservative, that is, to inflate the bootstrap quantile $t_{\alpha}^*$ by a small fraction, e.g. by $1\%$ to $1.01\,t^*_\alpha$. This simple procedure yields error bounds for the coverage probability of conservative bootstrap at as fast a rate as $\sqrt{(\log p)/n}$ under suitable conditions, so that not only the sample size requirement can be reduced to $\log p \ll n$ but also the overall convergence rate is nearly parametric. Furthermore, we improve the error bound for the coverage probability of the standard non-conservative bootstrap to $[(\log (np))^3 (\log p)^2/n]^{1/4}$ under general assumptions on data. These results are established for the empirical bootstrap and the multiplier bootstrap with third moment match. An improved coherent Lindeberg interpolation method, originally proposed in Deng and Zhang (2017), is developed to derive sharper comparison bounds, especially for the maxima.

==> backup.tex <==
{\sc Proof of Proposition \ref{prop:LP-empi}.} Let $u_n = M (n/(\log(np))^{1/4}$ and $a_n = \sqrt{n} \varepsilon /\log (np)$. Let $\widetilde{X}_{i,j} = X_{i,j}I\{|X_{i,j}| \le u_n \} - \mathbb{E} X_{i,j}I\{|X_{i,j}| \le u_n \}$, and $\{\widetilde{X}_{i,j}^*, 1\le i \le n \}$ be uniformly sampled from $\big\{ \widetilde{X}_{i,j}  - n^{-1} \sum_{k=1}^n \widetilde{X}_{k,j}, 1\le i \le n \big\}$. Let $\widetilde{T}_n = \max_j \sum_{i=1}^n \widetilde{X}_{i,j}/\sqrt{n}$ and $\widetilde{T}_n^* = \max_j \sum_{i=1}^n \widetilde{X}_{i,j}^*/\sqrt{n} $. It follows from the pseudo triangle inequality of the L\'evy-Prokhorov pre-distance in \eqref{triangle_inequality} that
\begin{align}\label{0-1-pf:LP-empi}
\eta_n^*(\varepsilon, t) &\le \sup_{t} \eta_n^*(\varepsilon/2, t; \widetilde{T}_n, \widetilde{T}_n^* ) + \mathbb{P} \Big[ \big\| \sum_{i=1}^n ( X_{i,j} - \widetilde{X}_{i, j})/\sqrt{n} \Big\|_{\infty} \ge \varepsilon/4 \Big]
\\ \nonumber
& \hspace{10.5em} + \mathbb{P}^* \Big[ \big\| \sum_{i=1}^n ( X_{i,j}^* - \widetilde{X}_{i, j}^* )/\sqrt{n} \Big\|_{\infty} \ge \varepsilon/4 \Big].
\end{align}	
We bound the above three quantities on the right-hand side when
\begin{align*}
\varepsilon \ge \varepsilon_0 = \sqrt{2\,C_{c_0, 2}} \{(\log (np))^3/n\}^{1/4} M
\end{align*}
for a sufficiently large constant $C_{c_0, 2}$ to be given later. This implies that $|\widetilde{X}_{i,j}| \le 2 u_n \le 2a_n = 2\sqrt{n} \varepsilon/\log (np)$. The case of $\varepsilon < \varepsilon_0$ will be considered in the end of the proof.

\smallskip
\noindent{$\bullet$ \it Step 1.} We bound $\displaystyle \eta_n^*(\varepsilon/2, t; \widetilde{T}_n, \widetilde{T}_n^*)$ through Theorem \ref{thm:DAT} in which we let $X_i = \widetilde{X}_i^0$ be an independent copy of $\widetilde{X}_i$, $Y_i = \widetilde{X}_i^*$, $m^*=4$ and $\mathbb{E}$ be $\mathbb{E}^* = \mathbb{E} [ \cdot | \widetilde{X}_i, 1\le i \le n]$. Note the variables $W_i$ in Theorem \eqref{thm:DAT} are taken to be fixed constant $4$. It follows from Theorem \ref{thm:DAT} that
\begin{align}\label{1-1-pf:LP-empi}
&\eta_n(\varepsilon/2, t; \widetilde{T}_n, \widetilde{T}_n^*) \le K_{n, 4}(\varepsilon/2) \min \bigg\{1, \frac{\omega_n \big( 11 \varepsilon/2; \widetilde{T}_n \big) }{ \big[ 1-K_{n, 4}(\varepsilon/2) \big]_+ } \bigg\}
\end{align}
where by Theorem \ref{thm:gAC},
\begin{align}\label{1-2-pf:LP-empi}
\displaystyle \omega_n(11\varepsilon/2; \widetilde{T}_n)  \le C_2 \bigg( \frac{(\log (np))^3 (\log p)^{1/2}}{n} \frac{M_4^4 }{\varepsilon^3 \overline{\sigma}} + \frac{\varepsilon}{\overline{\sigma}}\sqrt{\log p} \bigg).
\end{align}
We then bound $K_{n, 4}(\varepsilon/2)$. It follows from Bennett inequality that
\begin{align*}
& \sum_{m=1}^4
 \mathbb{P} \Bigg\{\bigg\| \frac{1}{n}\sum_{k=1}^n \Big(\widetilde{X}_k^{\otimes m} - \mathbb{E} \widetilde{X}_{k}^{\otimes m} \Big) \bigg\|_{\max} > (2 u_n)^mB_{n,m} \Bigg\}
\cr 
&\le \sum_{m=1}^4 (2p^m) \exp \bigg\{ - n \Big(\frac{M_4}{2 u_n}\Big)^{4 \wedge (2m)} \rho\Big((2 u_n/M_4)^{ 4 \wedge (2m)} B_{n,m}\Big) \bigg\}
\end{align*}
where $\rho(t) = (1+t)\log(1+t) - t$ satisfies $\rho(t) \ge t^2/(2K+2)$ when $t \le K$ for any $K > 2$. Recall $\log(np) \le  c_0  n$, we let $B_{n,m} = C_{c_0, 1} \big( \log (np)/n \big)^{3/4}$ for $m=1$ and $B_{n,m} = C_{c_0, 1} \log (np)/n$ for $m=2,3$ and $4$, where the constant $C_{c_0, 1}$ is large enough so that
\begin{align*}
\begin{cases}
\displaystyle \frac{4 C_{c_0, 1}^2}{ 8 C_{c_0, 1}  c_0 ^{1/4} + 2} \log(np) \ge \log(8np^{m+1}) & m=1,
\cr
\displaystyle \frac{\rho(2^4 C_{c_0, 1})}{2^4 } \log(np) \ge \log(8np^{m+1}) & m=2, 3, \hbox{ and } 4.
\end{cases}
\end{align*}
This implies that it holds with at least probability $1 - \sum_{m=1}^4 (2 p^m) \exp( - \log(8np^{m+1})) \ge 1 - (np)^{-1}$ that $\Big\| \frac{1}{n}\sum_{k=1}^n \Big(\widetilde{X}_k^{\otimes m} - \mathbb{E} \widetilde{X}_{k}^{\otimes m} \Big) \Big\|_{\max} \le (2 u_n)^mB_{n,m} $ for $m=1, \ldots, 4$. Hence, with probability at least $1-(np)^{-1}$,
\begin{align*}
d_n^{(m)} &:= \bigg\| \frac{1}{n} \sum_{k=1}^n \mathbb{E} \widetilde{X}_k^{\otimes m} - \frac{1}{n} \sum_{k=1}^n \Big(\widetilde{X}_k - \frac{1}{n}\sum_{\ell=1}^n \widetilde{X}_{\ell} \Big)^{\otimes m} \bigg\|_{\max}
\\ \nonumber
&= \Bigg\| \frac{1}{n}\sum_{k=1}^n \Big(\widetilde{X}_k^{\otimes m} - \frac{1}{n} \sum_{\ell =1}^n \mathbb{E} \widetilde{X}_{\ell}^{\otimes m} \Big)
+
\\ \nonumber
& \qquad \qquad \sum_{m_0 =1}^m {m \choose m_0} \mathrm{Sym}
\bigg[ \Big(- \frac{1}{n}\sum_{\ell=1}^n \widetilde{X}_{\ell}\Big)^{\otimes m_0} \otimes \Big( \frac{1}{n} \sum_{k=1}^n \widetilde{X}_k^{\otimes (m-m_0)}\Big)  \bigg] \Bigg\|_{\max}
\\ \nonumber
&\le \Bigg\| \frac{1}{n}\sum_{k=1}^n \Big(\widetilde{X}_k^{\otimes m} - \mathbb{E} \widetilde{X}_{k}^{\otimes m} \Big) \Bigg\|_{\max}
+ \sum_{m_0 =1}^m {m \choose m_0} \Bigg\|\frac{1}{n}\sum_{k=1}^n \Big( \widetilde{X}_{k} - \mathbb{E} \widetilde{X}_{k} \Big) \Bigg\|_{\infty}^{m_0} \times 
\\ \nonumber
& \qquad \Bigg( \bigg\| \frac{1}{n} \sum_{k=1}^n \Big(\widetilde{X}_k^{\otimes (m-m_0)} - \mathbb{E} \widetilde{X}_k^{\otimes (m-m_0)} \Big) \bigg\|_{\max} + \bigg\| \frac{1}{n} \sum_{k=1}^n \mathbb{E} \widetilde{X}_k^{\otimes (m-m_0)} \bigg\|_{\max} \Bigg)
\\ \nonumber
&\le (2 u_n)^m B_{n,m}
+ \sum_{m_0=1}^m {m \choose m_0} \big[ (2 u_n ) B_{n,1} \big]^{m_0} \times
\\ \nonumber
& \qquad \qquad \qquad \Big( (2 u_n)^{m-m_0} B_{n, m - m_0} + \big( M_4 \wedge (2 u_n) \big)^{m-m_0} \Big)
\\ \nonumber
&\le C_{c_0, m} u_n^m \log(np) /n,
\end{align*}
where $\mathrm{Sym}(A)$ denotes the symmetrization of tensor $A$ by taking the average over all permutations of the index of its elements, and then
\begin{align*}
K_{n,4}(\varepsilon/2) &\le  C_3 \bigg( \sum_{m=2}^{4} \frac{(\log (np) )^{m-1}}{n^{m/2-1}}  \frac{d_n^{(m)} }{\varepsilon^m} + \frac{(\log (np))^3 }{ n } \frac{M_4^4}{\varepsilon^4} \bigg)
\\ \nonumber
&\le C_{c_0, 2} \frac{(\log (np))^{3/2}}{n^{1/2} } \frac{M^2}{\varepsilon^2 }.
\end{align*}
As $\varepsilon \ge \varepsilon_0$ and $K_{n,4}(\varepsilon_0/2) \le 1/2$, it follows from \eqref{1-1-pf:LP-empi} and \eqref{1-2-pf:LP-empi} that with at least probability $1-(np)^{-1}$
\begin{align}\label{1-3-pf:LP-empi}
\eta_n(\varepsilon/2, t; \widetilde{T}_n, \widetilde{T}_n^*) &\le C_{c_0, 3} \min \Big\{\frac{(\log (np))^{3/2}}{n^{1/2}}\frac{M^2}{\varepsilon^2}, \frac{(\log (np))^{3/2}(\log p)^{1/2}}{n^{1/2}}\frac{M^2}{\varepsilon \overline{\sigma}}\Big\}
\\ \nonumber
&\le C_{c_0, 4} \min \Big\{\frac{(\log (np))^{3/2}}{n^{1/2}}\frac{M^2}{\varepsilon^2}, \frac{(\log (np))^{3/2}(\log p)^{1/2}}{n^{1/2}}\frac{M^2}{\varepsilon \overline{\sigma}}, 
\\ \nonumber 
&\hspace{14em} \Big(\frac{(\log(np))^3(\log p)^2}{n} \Big)^{1/4} \frac{M}{\overline{\sigma}}\Big\}.
\end{align}

\smallskip
\noindent{$\bullet$ \it Step 2.} We bound the other two terms on the right-hand side of \eqref{0-1-pf:LP-empi} using Lemmas 3 and 7 in \cite{deng2017beyond}, which yield that
\begin{align}\label{2-1-pf:LP-empi}
& \mathbb{P} \Big[ \big\| \sum_{i=1}^n ( X_{i,j} - \widetilde{X}_{i, j})/\sqrt{n} \Big\|_{\infty} \ge \varepsilon/4 \Big] \le (np)^{-1} + \mathbb{P} \big\{\| \boldsymbol{X} \|_{\max} \ge a_n \big\},
\\ \nonumber
& \mathbb{P} \Big\{ \mathbb{P}^* \Big[ \big\| \sum_{i=1}^n ( X_{i,j}^* - \widetilde{X}_{i, j}^* )/\sqrt{n} \Big\|_{\infty} \ge \varepsilon/4 \Big] > (np)^{-1} \Big\} \le (np)^{-1} + \mathbb{P} \big\{\| \boldsymbol{X} \|_{\max} \ge a_n \big\}.
\end{align}
Note that these Lemmas are applicable because $|\widetilde{X}_{i,j}| \le 2 u_n \le 2a_n$, which is essentially due to the condition $\varepsilon \ge \varepsilon_0$.

\smallskip
\noindent{$\bullet$ \it Step 3.} It follows from \eqref{0-1-pf:LP-empi}, \eqref{1-3-pf:LP-empi} and \eqref{2-1-pf:LP-empi} that for $\varepsilon \ge \varepsilon_0$,
\begin{align}\label{3-1-pf:LP-empi}
\eta_n^*(\varepsilon, t) &\le 2/(np) +  \mathbb{P} \big\{\| \boldsymbol{X} \|_{\max} \ge a_n \} + C_{c_0, 4} \min \bigg\{\frac{(\log (np))^{3/2}}{n^{1/2}}\frac{M^2}{\varepsilon^2}, 
\\ \nonumber 
&\hspace{4em} \frac{(\log (np))^{3/2}(\log p)^{1/2}}{n^{1/2}}\frac{M^2}{\varepsilon \overline{\sigma}}, \Big(\frac{(\log(np))^3(\log p)^2}{n} \Big)^{1/4} \frac{M}{\overline{\sigma}} \bigg\}
\end{align}	
with at least probability $1- 2/(np) -  \mathbb{P} \big\{\| \boldsymbol{X} \|_{\max} \ge a_n \}$. For $\varepsilon \le \varepsilon_0$, It follows from Theorem \ref{thm:gAC} and \eqref{3-2-pf:LP-empi} that
\begin{align}\label{3-2-pf:LP-empi}
\eta_n^*(\varepsilon, t) &\le \sup_{t} \big| \mathbb{P}\{T_n \le t\} - \mathbb{P}^* \{T_n^* \le t\} \big| 
\\ \nonumber
&\le \sup_t \eta_n^*(\varepsilon_0, t) + \omega_n(\varepsilon_0; T_n)
\\ \nonumber
&\le 2/(np) + 3 \mathbb{P} \Big\{\| \boldsymbol{X} \|_{\max} \ge \sqrt{2C_{c_0, 2}} u_n \Big\} + C_{c_0, 5} \Big(\frac{(\log (np))^3 (\log p)^2}{n} \Big)^{1/4} \frac{M}{\overline{\sigma}}
\end{align}
with at least probability $\displaystyle 1 - 2/(np) -  \mathbb{P} \big\{\| \boldsymbol{X} \|_{\max} \ge \sqrt{2C_{c_0, 2}} u_n \big\}$.
The final conclusion \eqref{1-prop:LP-empi} follows from \eqref{3-1-pf:LP-empi} and \eqref{3-2-pf:LP-empi} with proper rescaling on constant coefficients. The proof is complete. $\hfill\square$

\begin{proposition}\label{prop:LP-multi}
Let $q_0(M, \varepsilon) =  \mathbb{P} \Big\{\| \boldsymbol{X} \|_{\max}> \max \big[ M(n/\log (np) )^{1/4}, \sqrt{n} \varepsilon /\log (n p) \big]\Big\}$ with $M \ge M_4$. Suppose there exists a fixed constant $c_0$ s.t. $\log(np) \le c_0 n$. Then, with at least probability $1 - 2/(np) - q_0(M, \varepsilon)$,
\begin{align}\label{1-prop:LP-multi}
\sup_t \eta_n^*(\varepsilon, t)   &\le C_{c_0} \min \bigg\{\frac{(\log (np))^{3/2}}{n^{1/2}}\frac{M^2}{\varepsilon^2}, \frac{(\log (np))^{3/2}(\log p)^{1/2}}{n^{1/2}}\frac{M^2}{\varepsilon \overline{\sigma}},
\\ \nonumber 
&\hspace{10em} \Big(\frac{(\log(np))^3(\log p)^2}{n} \Big)^{1/4} \frac{M}{\overline{\sigma}} \bigg\} + 2/(np) +  3q_0(M, \varepsilon)
\end{align}
\end{proposition}

==> conservative v8/backup.tex <==
{\sc Proof of Proposition \ref{prop:LP-empi}.} Let $u_n = M (n/(\log(np))^{1/4}$ and $a_n = \sqrt{n} \varepsilon /\log (np)$. Let $\widetilde{X}_{i,j} = X_{i,j}I\{|X_{i,j}| \le u_n \} - \mathbb{E} X_{i,j}I\{|X_{i,j}| \le u_n \}$, and $\{\widetilde{X}_{i,j}^*, 1\le i \le n \}$ be uniformly sampled from $\big\{ \widetilde{X}_{i,j}  - n^{-1} \sum_{k=1}^n \widetilde{X}_{k,j}, 1\le i \le n \big\}$. Let $\widetilde{T}_n = \max_j \sum_{i=1}^n \widetilde{X}_{i,j}/\sqrt{n}$ and $\widetilde{T}_n^* = \max_j \sum_{i=1}^n \widetilde{X}_{i,j}^*/\sqrt{n} $. It follows from the pseudo triangle inequality of the L\'evy-Prokhorov pre-distance in \eqref{triangle_inequality} that
\begin{align}\label{0-1-pf:LP-empi}
\eta_n^*(\varepsilon, t) &\le \sup_{t} \eta_n^*(\varepsilon/2, t; \widetilde{T}_n, \widetilde{T}_n^* ) + \mathbb{P} \Big[ \big\| \sum_{i=1}^n ( X_{i,j} - \widetilde{X}_{i, j})/\sqrt{n} \Big\|_{\infty} \ge \varepsilon/4 \Big]
\\ \nonumber
& \hspace{10.5em} + \mathbb{P}^* \Big[ \big\| \sum_{i=1}^n ( X_{i,j}^* - \widetilde{X}_{i, j}^* )/\sqrt{n} \Big\|_{\infty} \ge \varepsilon/4 \Big].
\end{align}	
We bound the above three quantities on the right-hand side when
\begin{align*}
\varepsilon \ge \varepsilon_0 = \sqrt{2\,C_{c_0, 2}} \{(\log (np))^3/n\}^{1/4} M
\end{align*}
for a sufficiently large constant $C_{c_0, 2}$ to be given later. This implies that $|\widetilde{X}_{i,j}| \le 2 u_n \le 2a_n = 2\sqrt{n} \varepsilon/\log (np)$. The case of $\varepsilon < \varepsilon_0$ will be considered in the end of the proof.

\smallskip
\noindent{$\bullet$ \it Step 1.} We bound $\displaystyle \eta_n^*(\varepsilon/2, t; \widetilde{T}_n, \widetilde{T}_n^*)$ through Theorem \ref{thm:DAT} in which we let $X_i = \widetilde{X}_i^0$ be an independent copy of $\widetilde{X}_i$, $Y_i = \widetilde{X}_i^*$, $m^*=4$ and $\mathbb{E}$ be $\mathbb{E}^* = \mathbb{E} [ \cdot | \widetilde{X}_i, 1\le i \le n]$. Note the variables $W_i$ in Theorem \eqref{thm:DAT} are taken to be fixed constant $4$. It follows from Theorem \ref{thm:DAT} that
\begin{align}\label{1-1-pf:LP-empi}
&\eta_n(\varepsilon/2, t; \widetilde{T}_n, \widetilde{T}_n^*) \le K_{n, 4}(\varepsilon/2) \min \bigg\{1, \frac{\omega_n \big( 11 \varepsilon/2; \widetilde{T}_n \big) }{ \big[ 1-K_{n, 4}(\varepsilon/2) \big]_+ } \bigg\}
\end{align}
where by Theorem \ref{thm:gAC},
\begin{align}\label{1-2-pf:LP-empi}
\displaystyle \omega_n(11\varepsilon/2; \widetilde{T}_n)  \le C_2 \bigg( \frac{(\log (np))^3 (\log p)^{1/2}}{n} \frac{M_4^4 }{\varepsilon^3 \overline{\sigma}} + \frac{\varepsilon}{\overline{\sigma}}\sqrt{\log p} \bigg).
\end{align}
We then bound $K_{n, 4}(\varepsilon/2)$. It follows from Bennett inequality that
\begin{align*}
& \sum_{m=1}^4
 \mathbb{P} \Bigg\{\bigg\| \frac{1}{n}\sum_{k=1}^n \Big(\widetilde{X}_k^{\otimes m} - \mathbb{E} \widetilde{X}_{k}^{\otimes m} \Big) \bigg\|_{\max} > (2 u_n)^mB_{n,m} \Bigg\}
\cr 
&\le \sum_{m=1}^4 (2p^m) \exp \bigg\{ - n \Big(\frac{M_4}{2 u_n}\Big)^{4 \wedge (2m)} \rho\Big((2 u_n/M_4)^{ 4 \wedge (2m)} B_{n,m}\Big) \bigg\}
\end{align*}
where $\rho(t) = (1+t)\log(1+t) - t$ satisfies $\rho(t) \ge t^2/(2K+2)$ when $t \le K$ for any $K > 2$. Recall $\log(np) \le  c_0  n$, we let $B_{n,m} = C_{c_0, 1} \big( \log (np)/n \big)^{3/4}$ for $m=1$ and $B_{n,m} = C_{c_0, 1} \log (np)/n$ for $m=2,3$ and $4$, where the constant $C_{c_0, 1}$ is large enough so that
\begin{align*}
\begin{cases}
\displaystyle \frac{4 C_{c_0, 1}^2}{ 8 C_{c_0, 1}  c_0 ^{1/4} + 2} \log(np) \ge \log(8np^{m+1}) & m=1,
\cr
\displaystyle \frac{\rho(2^4 C_{c_0, 1})}{2^4 } \log(np) \ge \log(8np^{m+1}) & m=2, 3, \hbox{ and } 4.
\end{cases}
\end{align*}
This implies that it holds with at least probability $1 - \sum_{m=1}^4 (2 p^m) \exp( - \log(8np^{m+1})) \ge 1 - (np)^{-1}$ that $\Big\| \frac{1}{n}\sum_{k=1}^n \Big(\widetilde{X}_k^{\otimes m} - \mathbb{E} \widetilde{X}_{k}^{\otimes m} \Big) \Big\|_{\max} \le (2 u_n)^mB_{n,m} $ for $m=1, \ldots, 4$. Hence, with probability at least $1-(np)^{-1}$,
\begin{align*}
d_n^{(m)} &:= \bigg\| \frac{1}{n} \sum_{k=1}^n \mathbb{E} \widetilde{X}_k^{\otimes m} - \frac{1}{n} \sum_{k=1}^n \Big(\widetilde{X}_k - \frac{1}{n}\sum_{\ell=1}^n \widetilde{X}_{\ell} \Big)^{\otimes m} \bigg\|_{\max}
\\ \nonumber
&= \Bigg\| \frac{1}{n}\sum_{k=1}^n \Big(\widetilde{X}_k^{\otimes m} - \frac{1}{n} \sum_{\ell =1}^n \mathbb{E} \widetilde{X}_{\ell}^{\otimes m} \Big)
+
\\ \nonumber
& \qquad \qquad \sum_{m_0 =1}^m {m \choose m_0} \mathrm{Sym}
\bigg[ \Big(- \frac{1}{n}\sum_{\ell=1}^n \widetilde{X}_{\ell}\Big)^{\otimes m_0} \otimes \Big( \frac{1}{n} \sum_{k=1}^n \widetilde{X}_k^{\otimes (m-m_0)}\Big)  \bigg] \Bigg\|_{\max}
\\ \nonumber
&\le \Bigg\| \frac{1}{n}\sum_{k=1}^n \Big(\widetilde{X}_k^{\otimes m} - \mathbb{E} \widetilde{X}_{k}^{\otimes m} \Big) \Bigg\|_{\max}
+ \sum_{m_0 =1}^m {m \choose m_0} \Bigg\|\frac{1}{n}\sum_{k=1}^n \Big( \widetilde{X}_{k} - \mathbb{E} \widetilde{X}_{k} \Big) \Bigg\|_{\infty}^{m_0} \times 
\\ \nonumber
& \qquad \Bigg( \bigg\| \frac{1}{n} \sum_{k=1}^n \Big(\widetilde{X}_k^{\otimes (m-m_0)} - \mathbb{E} \widetilde{X}_k^{\otimes (m-m_0)} \Big) \bigg\|_{\max} + \bigg\| \frac{1}{n} \sum_{k=1}^n \mathbb{E} \widetilde{X}_k^{\otimes (m-m_0)} \bigg\|_{\max} \Bigg)
\\ \nonumber
&\le (2 u_n)^m B_{n,m}
+ \sum_{m_0=1}^m {m \choose m_0} \big[ (2 u_n ) B_{n,1} \big]^{m_0} \times
\\ \nonumber
& \qquad \qquad \qquad \Big( (2 u_n)^{m-m_0} B_{n, m - m_0} + \big( M_4 \wedge (2 u_n) \big)^{m-m_0} \Big)
\\ \nonumber
&\le C_{c_0, m} u_n^m \log(np) /n,
\end{align*}
where $\mathrm{Sym}(A)$ denotes the symmetrization of tensor $A$ by taking the average over all permutations of the index of its elements, and then
\begin{align*}
K_{n,4}(\varepsilon/2) &\le  C_3 \bigg( \sum_{m=2}^{4} \frac{(\log (np) )^{m-1}}{n^{m/2-1}}  \frac{d_n^{(m)} }{\varepsilon^m} + \frac{(\log (np))^3 }{ n } \frac{M_4^4}{\varepsilon^4} \bigg)
\\ \nonumber
&\le C_{c_0, 2} \frac{(\log (np))^{3/2}}{n^{1/2} } \frac{M^2}{\varepsilon^2 }.
\end{align*}
As $\varepsilon \ge \varepsilon_0$ and $K_{n,4}(\varepsilon_0/2) \le 1/2$, it follows from \eqref{1-1-pf:LP-empi} and \eqref{1-2-pf:LP-empi} that with at least probability $1-(np)^{-1}$
\begin{align}\label{1-3-pf:LP-empi}
\eta_n(\varepsilon/2, t; \widetilde{T}_n, \widetilde{T}_n^*) &\le C_{c_0, 3} \min \Big\{\frac{(\log (np))^{3/2}}{n^{1/2}}\frac{M^2}{\varepsilon^2}, \frac{(\log (np))^{3/2}(\log p)^{1/2}}{n^{1/2}}\frac{M^2}{\varepsilon \overline{\sigma}}\Big\}
\\ \nonumber
&\le C_{c_0, 4} \min \Big\{\frac{(\log (np))^{3/2}}{n^{1/2}}\frac{M^2}{\varepsilon^2}, \frac{(\log (np))^{3/2}(\log p)^{1/2}}{n^{1/2}}\frac{M^2}{\varepsilon \overline{\sigma}}, 
\\ \nonumber 
&\hspace{14em} \Big(\frac{(\log(np))^3(\log p)^2}{n} \Big)^{1/4} \frac{M}{\overline{\sigma}}\Big\}.
\end{align}

\smallskip
\noindent{$\bullet$ \it Step 2.} We bound the other two terms on the right-hand side of \eqref{0-1-pf:LP-empi} using Lemmas 3 and 7 in \cite{deng2017beyond}, which yield that
\begin{align}\label{2-1-pf:LP-empi}
& \mathbb{P} \Big[ \big\| \sum_{i=1}^n ( X_{i,j} - \widetilde{X}_{i, j})/\sqrt{n} \Big\|_{\infty} \ge \varepsilon/4 \Big] \le (np)^{-1} + \mathbb{P} \big\{\| \boldsymbol{X} \|_{\max} \ge a_n \big\},
\\ \nonumber
& \mathbb{P} \Big\{ \mathbb{P}^* \Big[ \big\| \sum_{i=1}^n ( X_{i,j}^* - \widetilde{X}_{i, j}^* )/\sqrt{n} \Big\|_{\infty} \ge \varepsilon/4 \Big] > (np)^{-1} \Big\} \le (np)^{-1} + \mathbb{P} \big\{\| \boldsymbol{X} \|_{\max} \ge a_n \big\}.
\end{align}
Note that these Lemmas are applicable because $|\widetilde{X}_{i,j}| \le 2 u_n \le 2a_n$, which is essentially due to the condition $\varepsilon \ge \varepsilon_0$.

\smallskip
\noindent{$\bullet$ \it Step 3.} It follows from \eqref{0-1-pf:LP-empi}, \eqref{1-3-pf:LP-empi} and \eqref{2-1-pf:LP-empi} that for $\varepsilon \ge \varepsilon_0$,
\begin{align}\label{3-1-pf:LP-empi}
\eta_n^*(\varepsilon, t) &\le 2/(np) +  \mathbb{P} \big\{\| \boldsymbol{X} \|_{\max} \ge a_n \} + C_{c_0, 4} \min \bigg\{\frac{(\log (np))^{3/2}}{n^{1/2}}\frac{M^2}{\varepsilon^2}, 
\\ \nonumber 
&\hspace{4em} \frac{(\log (np))^{3/2}(\log p)^{1/2}}{n^{1/2}}\frac{M^2}{\varepsilon \overline{\sigma}}, \Big(\frac{(\log(np))^3(\log p)^2}{n} \Big)^{1/4} \frac{M}{\overline{\sigma}} \bigg\}
\end{align}	
with at least probability $1- 2/(np) -  \mathbb{P} \big\{\| \boldsymbol{X} \|_{\max} \ge a_n \}$. For $\varepsilon \le \varepsilon_0$, It follows from Theorem \ref{thm:gAC} and \eqref{3-2-pf:LP-empi} that
\begin{align}\label{3-2-pf:LP-empi}
\eta_n^*(\varepsilon, t) &\le \sup_{t} \big| \mathbb{P}\{T_n \le t\} - \mathbb{P}^* \{T_n^* \le t\} \big| 
\\ \nonumber
&\le \sup_t \eta_n^*(\varepsilon_0, t) + \omega_n(\varepsilon_0; T_n)
\\ \nonumber
&\le 2/(np) + 3 \mathbb{P} \Big\{\| \boldsymbol{X} \|_{\max} \ge \sqrt{2C_{c_0, 2}} u_n \Big\} + C_{c_0, 5} \Big(\frac{(\log (np))^3 (\log p)^2}{n} \Big)^{1/4} \frac{M}{\overline{\sigma}}
\end{align}
with at least probability $\displaystyle 1 - 2/(np) -  \mathbb{P} \big\{\| \boldsymbol{X} \|_{\max} \ge \sqrt{2C_{c_0, 2}} u_n \big\}$.
The final conclusion \eqref{1-prop:LP-empi} follows from \eqref{3-1-pf:LP-empi} and \eqref{3-2-pf:LP-empi} with proper rescaling on constant coefficients. The proof is complete. $\hfill\square$

\begin{proposition}\label{prop:LP-multi}
Let $q_0(M, \varepsilon) =  \mathbb{P} \Big\{\| \boldsymbol{X} \|_{\max}> \max \big[ M(n/\log (np) )^{1/4}, \sqrt{n} \varepsilon /\log (n p) \big]\Big\}$ with $M \ge M_4$. Suppose there exists a fixed constant $c_0$ s.t. $\log(np) \le c_0 n$. Then, with at least probability $1 - 2/(np) - q_0(M, \varepsilon)$,
\begin{align}\label{1-prop:LP-multi}
\sup_t \eta_n^*(\varepsilon, t)   &\le C_{c_0} \min \bigg\{\frac{(\log (np))^{3/2}}{n^{1/2}}\frac{M^2}{\varepsilon^2}, \frac{(\log (np))^{3/2}(\log p)^{1/2}}{n^{1/2}}\frac{M^2}{\varepsilon \overline{\sigma}},
\\ \nonumber 
&\hspace{10em} \Big(\frac{(\log(np))^3(\log p)^2}{n} \Big)^{1/4} \frac{M}{\overline{\sigma}} \bigg\} + 2/(np) +  3q_0(M, \varepsilon)
\end{align}
\end{proposition}
